Experience Report: Teaching Code Analysis and Verification Using Frama-C

Formal methods provide systematic and rigorous techniques for software development. We strongly believe that they must be taught in computer science curricula. In this paper we present the pedagogic rationale and the concrete implementation of two courses on the use of formal methods, sharing some material. These courses promote the usage of formal verification to ensure safety and security of software, exemplified in the domain of the Internet of Things.

==> eptcsdata.tex <==
\providecommand{\firstpage}{69}
\providecommand{\publicationstatus}{M. Gleirscher, J.v.d. Pol, J. Woodcock (Eds.):\\First Workshop on Applicable Formal Methods (AppFM 2021).\\
EPTCS 349, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.349.5}{10.4204/EPTCS.349.5}}
\pdfoutput=1

